Evidence for $B^0 \to p\bar{\Sigma}^0\pi^-$ at Belle

We search for the $B^0\to p\bar{\Sigma}^0\pi^-$ decay with $\bar{\Sigma}^0 \to \bar{\Lambda}\gamma$, where the $\gamma$ is not measured, using a data sample corresponding to an integrated luminosity of 711 $\rm{fb^{-1}}$ which contains 772 $\times$ $10^{6}$ $B\bar{B}$ pairs, collected around the $\Upsilon$(4S) resonance with the Belle detector at the KEKB asymmetric-energy $e^{+}e^{-}$ collider. We measure for the first time the $B^0\to p\bar{\Sigma}^0\pi^-$ branching fraction to be $\mathcal{B}(B^0 \to p \bar\Sigma^0 \pi^-) = (1.17^{+0.43}_{-0.40}(\text{stat})\pm 0.07(\text{syst})) \times 10^{-6}$ with a significance of $3.0\sigma$. We simultaneously measure the branching fraction for the related channel $B^{0}\to p\bar{\Lambda}\pi^{-}$ with much improved precision.

==> pub648-orcid.tex <==
%%% Paper:    B0 to p Sigma0-bar pi-
%%% Journal:  Physical Review D
%%% Contacts: C.Y. Chang, M.Z. Wang
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{pub648-orcid} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
  \author{C.-Y.~Chang\,\orcidlink{0000-0003-1614-1708}} % 11983
  \author{M.-Z.~Wang\,\orcidlink{0000-0002-0979-8341}} % 2074
  \author{I.~Adachi\,\orcidlink{0000-0003-2287-0173}} % 2590
% \author{K.~Adamczyk\,\orcidlink{0000-0001-6208-0876}} % 2239
% \author{J.~K.~Ahn\,\orcidlink{0000-0002-5795-2243}} % 7423
  \author{H.~Aihara\,\orcidlink{0000-0002-1907-5964}} % 2223
  \author{S.~Al~Said\,\orcidlink{0000-0002-4895-3869}} % 6823
  \author{D.~M.~Asner\,\orcidlink{0000-0002-1586-5790}} % 4684
  \author{H.~Atmacan\,\orcidlink{0000-0003-2435-501X}} % 2538
% \author{V.~Aulchenko\,\orcidlink{0000-0002-5394-4406}} % 8183
  \author{T.~Aushev\,\orcidlink{0000-0002-6347-7055}} % 3747
  \author{R.~Ayad\,\orcidlink{0000-0003-3466-9290}} % 3766
% \author{T.~Aziz\,\orcidlink{-}} % 3523
  \author{V.~Babu\,\orcidlink{0000-0003-0419-6912}} % 5623
% \author{S.~Bahinipati\,\orcidlink{0000-0002-3744-5332}} % 2332
% \author{A.~M.~Bakich\,\orcidlink{0000-0001-8315-4854}} % 2115
% \author{Y.~Ban\,\orcidlink{-}} % 3503
  \author{Sw.~Banerjee\,\orcidlink{0000-0001-8852-2409}} % 8603
% \author{E.~Barberio\,\orcidlink{-}} % -229
% \author{M.~Barrett\,\orcidlink{0000-0002-2095-603X}} % 2180
  \author{M.~Bauer\,\orcidlink{0000-0002-0953-7387}} % 9863
  \author{P.~Behera\,\orcidlink{0000-0002-1527-2266}} % 4204
  \author{K.~Belous\,\orcidlink{0000-0003-0014-2589}} % 2329
  \author{J.~Bennett\,\orcidlink{0000-0002-5440-2668}} % 2454
  \author{F.~Bernlochner\,\orcidlink{0000-0001-8153-2719}} % 2282
  \author{M.~Bessner\,\orcidlink{0000-0003-1776-0439}} % 3783
% \author{D.~Besson\,\orcidlink{-}} % 3585
% \author{V.~Bhardwaj\,\orcidlink{0000-0001-8857-8621}} % 2228
% \author{B.~Bhuyan\,\orcidlink{0000-0001-6254-3594}} % 2097
  \author{T.~Bilka\,\orcidlink{0000-0003-1449-6986}} % 2484
% \author{S.~Bilokin\,\orcidlink{0000-0003-0017-6260}} % 3623
  \author{D.~Biswas\,\orcidlink{0000-0002-7543-3471}} % 8703
% \author{T.~Bloomfield\,\orcidlink{0000-0001-9288-5069}} % 2418
  \author{A.~Bobrov\,\orcidlink{0000-0001-5735-8386}} % 2294
  \author{D.~Bodrov\,\orcidlink{0000-0001-5279-4787}} % 9643
% \author{A.~Bondar\,\orcidlink{0000-0002-5089-5338}} % 4643
  \author{G.~Bonvicini\,\orcidlink{0000-0003-4861-7918}} % 2095
  \author{J.~Borah\,\orcidlink{0000-0003-2990-1913}} % 7083
  \author{A.~Bozek\,\orcidlink{0000-0002-5915-1319}} % 2303
  \author{M.~Bra\v{c}ko\,\orcidlink{0000-0002-2495-0524}} % 2425
  \author{P.~Branchini\,\orcidlink{0000-0002-2270-9673}} % 2577
  \author{T.~E.~Browder\,\orcidlink{0000-0001-7357-9007}} % 2560
  \author{A.~Budano\,\orcidlink{0000-0002-0856-1131}} % 2171
  \author{M.~Campajola\,\orcidlink{0000-0003-2518-7134}} % 5223
  \author{L.~Cao\,\orcidlink{0000-0001-8332-5668}} % 2099
  \author{D.~\v{C}ervenkov\,\orcidlink{0000-0002-1865-741X}} % 2078
  \author{M.-C.~Chang\,\orcidlink{0000-0002-8650-6058}} % 2827
% \author{P.~Chang\,\orcidlink{0000-0003-4064-388X}} % 2542
% \author{V.~Chekelian\,\orcidlink{0000-0001-8860-8288}} % 2167
% \author{A.~Chen\,\orcidlink{0000-0002-8544-9274}} % -284
% \author{C.~Chen\,\orcidlink{0000-0003-1589-9955}} % 12803
% \author{Y.~Chen\,\orcidlink{0000-0002-2057-1076}} % 2576
% \author{Y.-T.~Chen\,\orcidlink{0000-0003-2639-2850}} % 2884
  \author{B.~G.~Cheon\,\orcidlink{0000-0002-8803-4429}} % 2173
  \author{K.~Chilikin\,\orcidlink{0000-0001-7620-2053}} % 2308
  \author{H.~E.~Cho\,\orcidlink{0000-0002-7008-3759}} % 2182
  \author{K.~Cho\,\orcidlink{0000-0003-1705-7399}} % 2516
  \author{S.-J.~Cho\,\orcidlink{0000-0002-1673-5664}} % 2723
  \author{S.-K.~Choi\,\orcidlink{0000-0003-2747-8277}} % 2364
  \author{Y.~Choi\,\orcidlink{0000-0003-3499-7948}} % -405
  \author{S.~Choudhury\,\orcidlink{0000-0001-9841-0216}} % 2206
  \author{D.~Cinabro\,\orcidlink{0000-0001-7347-6585}} % 2092
% \author{J.~Cochran\,\orcidlink{0000-0002-1492-914X}} % 12604
% \author{S.~Cunliffe\,\orcidlink{0000-0003-0167-8641}} % 2272
% \author{T.~Czank\,\orcidlink{0000-0001-6621-3373}} % 2254
  \author{S.~Das\,\orcidlink{0000-0001-6857-966X}} % 9163
% \author{N.~Dash\,\orcidlink{0000-0003-2172-3534}} % 2601
% \author{G.~de~Marino\,\orcidlink{0000-0002-6509-7793}} % 8364
  \author{G.~De~Nardo\,\orcidlink{0000-0002-2047-9675}} % 2459
  \author{G.~De~Pietro\,\orcidlink{0000-0001-8442-107X}} % 2528
  \author{R.~Dhamija\,\orcidlink{0000-0001-7052-3163}} % 9465
  \author{F.~Di~Capua\,\orcidlink{0000-0001-9076-5936}} % 2065
% \author{J.~Dingfelder\,\orcidlink{0000-0001-5767-2121}} % 2151
  \author{Z.~Dole\v{z}al\,\orcidlink{0000-0002-5662-3675}} % 2319
  \author{T.~V.~Dong\,\orcidlink{0000-0003-3043-1939}} % 2215
% \author{D.~Dossett\,\orcidlink{0000-0002-5670-5582}} % 2574
  \author{S.~Dubey\,\orcidlink{0000-0002-1345-0970}} % 11063
  \author{P.~Ecker\,\orcidlink{0000-0002-6817-6868}} % 5563
% \author{D.~Epifanov\,\orcidlink{0000-0001-8656-2693}} % 2551
% \author{M.~Feindt\,\orcidlink{-}} % -532
  \author{T.~Ferber\,\orcidlink{0000-0002-6849-0427}} % 2482
  \author{D.~Ferlewicz\,\orcidlink{0000-0002-4374-1234}} % 2073
% \author{A.~Frey\,\orcidlink{0000-0001-7470-3874}} % 2150
  \author{B.~G.~Fulsom\,\orcidlink{0000-0002-5862-9739}} % 2563
% \author{R.~Garg\,\orcidlink{0000-0002-7406-4707}} % 2213
  \author{V.~Gaur\,\orcidlink{0000-0002-8880-6134}} % 2413
% \author{N.~Gabyshev\,\orcidlink{0000-0002-8593-6857}} % 2510
  \author{A.~Garmash\,\orcidlink{0000-0003-2599-1405}} % 2161
  \author{A.~Giri\,\orcidlink{0000-0002-8895-0128}} % 2106
  \author{P.~Goldenzweig\,\orcidlink{0000-0001-8785-847X}} % 2345
% \author{B.~Golob\,\orcidlink{0000-0001-9632-5616}} % 3703
% \author{G.~Gong\,\orcidlink{0000-0001-7192-1833}} % 2727
  \author{E.~Graziani\,\orcidlink{0000-0001-8602-5652}} % 2342
% \author{D.~Greenwald\,\orcidlink{0000-0001-6964-8399}} % 2686
  \author{T.~Gu\,\orcidlink{0000-0002-1470-6536}} % 14283
  \author{Y.~Guan\,\orcidlink{0000-0002-5541-2278}} % 2514
  \author{K.~Gudkova\,\orcidlink{0000-0002-5858-3187}} % 10504
  \author{C.~Hadjivasiliou\,\orcidlink{0000-0002-2234-0001}} % 9503
% \author{H.~Haigh\,\orcidlink{0000-0003-1567-0907}} % 16744
  \author{S.~Halder\,\orcidlink{0000-0002-6280-494X}} % 4743
% \author{X.~Han\,\orcidlink{0000-0003-1656-9413}} % 2589
% \author{K.~Hara\,\orcidlink{0000-0002-5361-1871}} % 2462
  \author{T.~Hara\,\orcidlink{0000-0002-4321-0417}} % 2523
% \author{O.~Hartbrich\,\orcidlink{0000-0001-7741-4381}} % 2158
  \author{K.~Hayasaka\,\orcidlink{0000-0002-6347-433X}} % 2330
  \author{H.~Hayashii\,\orcidlink{0000-0002-5138-5903}} % 2455
  \author{S.~Hazra\,\orcidlink{0000-0001-6954-9593}} % 7663
  \author{M.~T.~Hedges\,\orcidlink{0000-0001-6504-1872}} % 2265
  \author{D.~Herrmann\,\orcidlink{0000-0001-9772-9989}} % -565
% \author{M.~Hern\'{a}ndez~Villanueva\,\orcidlink{0000-0002-6322-5587}} % 2466
% \author{T.~Higuchi\,\orcidlink{0000-0002-7761-3505}} % 2485
% \author{H.~Hirata\,\orcidlink{0000-0001-9005-4616}} % 2070
  \author{W.-S.~Hou\,\orcidlink{0000-0002-4260-5118}} % -288
  \author{C.-L.~Hsu\,\orcidlink{0000-0002-1641-430X}} % 2299
% \author{K.~Huang\,\orcidlink{0000-0001-9342-7406}} % 2389
% \author{T.~Iijima\,\orcidlink{0000-0002-4271-711X}} % 2446
  \author{K.~Inami\,\orcidlink{0000-0003-2765-7072}} % 2323
% \author{G.~Inguglia\,\orcidlink{0000-0003-0331-8279}} % 2500
  \author{N.~Ipsita\,\orcidlink{0000-0002-2927-3366}} % 12223
  \author{A.~Ishikawa\,\orcidlink{0000-0002-3561-5633}} % 2281
  \author{R.~Itoh\,\orcidlink{0000-0003-1590-0266}} % 2487
  \author{M.~Iwasaki\,\orcidlink{0000-0002-9402-7559}} % 2360
  \author{Y.~Iwasaki\,\orcidlink{0000-0001-7261-2557}} % 2229
% \author{S.~Iwata\,\orcidlink{0009-0005-5017-8098}} % 4323
  \author{W.~W.~Jacobs\,\orcidlink{0000-0002-9996-6336}} % 2322
% \author{E.-J.~Jang\,\orcidlink{0000-0002-1935-9887}} % 6744
% \author{H.~B.~Jeon\,\orcidlink{0000-0002-0857-0353}} % 2170
% \author{Q.~P.~Ji\,\orcidlink{0000-0003-2963-2565}} % 16243
  \author{S.~Jia\,\orcidlink{0000-0001-8176-8545}} % 2457
  \author{Y.~Jin\,\orcidlink{0000-0002-7323-0830}} % 2105
  \author{K.~K.~Joo\,\orcidlink{0000-0002-5515-0087}} % 4224
% \author{J.~Kahn\,\orcidlink{0000-0002-8517-2359}} % 2448
% \author{H.~Kakuno\,\orcidlink{0000-0002-9957-6055}} % 2391
% \author{D.~Kalita\,\orcidlink{0000-0003-3054-1222}} % 2220
  \author{A.~B.~Kaliyar\,\orcidlink{0000-0002-2211-619X}} % 7344
% \author{K.~H.~Kang\,\orcidlink{0000-0002-6816-0751}} % 2283
% \author{S.~Kang\,\orcidlink{0000-0002-5320-7043}} % 12683
% \author{P.~Kapusta\,\orcidlink{0000-0003-1235-1935}} % 6663
% \author{G.~Karyan\,\orcidlink{0000-0001-5365-3716}} % 2550
% \author{Y.~Kato\,\orcidlink{0000-0001-6314-4288}} % 2549
% \author{H.~Kawai\,\orcidlink{-}} % 4344
  \author{T.~Kawasaki\,\orcidlink{0000-0002-4089-5238}} % 4363
% \author{H.~Kichimi\,\orcidlink{0000-0003-0534-4710}} % 2233
  \author{C.~Kiesling\,\orcidlink{0000-0002-2209-535X}} % 2168
  \author{C.~H.~Kim\,\orcidlink{0000-0002-5743-7698}} % 2358
  \author{D.~Y.~Kim\,\orcidlink{0000-0001-8125-9070}} % 2315
% \author{H.~J.~Kim\,\orcidlink{0000-0001-9787-4684}} % 4863
  \author{K.-H.~Kim\,\orcidlink{0000-0002-4659-1112}} % 2118
% \author{K.~T.~Kim\,\orcidlink{0000-0003-2884-6772}} % 2409
% \author{S.~K.~Kim\,\orcidlink{-}} % 3823
% \author{Y.~J.~Kim\,\orcidlink{0000-0001-9511-9634}} % 2403
  \author{Y.-K.~Kim\,\orcidlink{0000-0002-9695-8103}} % 2379
% \author{T.~D.~Kimmel\,\orcidlink{0000-0002-9743-8249}} % 2241
% \author{H.~Kindo\,\orcidlink{0000-0002-6756-3591}} % 2195
  \author{K.~Kinoshita\,\orcidlink{0000-0001-7175-4182}} % 2318
% \author{C.~Kleinwort\,\orcidlink{0000-0002-9017-9504}} % 2499
  \author{P.~Kody\v{s}\,\orcidlink{0000-0002-8644-2349}} % 2407
% \author{I.~Komarov\,\orcidlink{0000-0001-6282-1881}} % 2210
  \author{T.~Konno\,\orcidlink{0000-0003-2487-8080}} % 2490
  \author{A.~Korobov\,\orcidlink{0000-0001-5959-8172}} % 4185
  \author{S.~Korpar\,\orcidlink{0000-0003-0971-0968}} % 2475
  \author{E.~Kovalenko\,\orcidlink{0000-0001-8084-1931}} % 3884
  \author{P.~Kri\v{z}an\,\orcidlink{0000-0002-4967-7675}} % 2474
% \author{R.~Kroeger\,\orcidlink{-}} % 2242
% \author{J.-F.~Krohn\,\orcidlink{0000-0002-5001-0675}} % 2502
  \author{P.~Krokovny\,\orcidlink{0000-0002-1236-4667}} % 2575
  \author{T.~Kuhr\,\orcidlink{0000-0001-6251-8049}} % 2486
  \author{M.~Kumar\,\orcidlink{0000-0002-6627-9708}} % 2744
% \author{R.~Kumar\,\orcidlink{0000-0002-6277-2626}} % 2189
  \author{K.~Kumara\,\orcidlink{0000-0003-1572-5365}} % 2257
% \author{T.~Kumita\,\orcidlink{0000-0001-7572-4538}} % 4083
% \author{E.~Kurihara\,\orcidlink{-}} % -95
  \author{A.~Kuzmin\,\orcidlink{0000-0002-7011-5044}} % 2520
% \author{P.~Kvasni\v{c}ka\,\orcidlink{0000-0001-6281-0648}} % 2184
  \author{Y.-J.~Kwon\,\orcidlink{0000-0001-9448-5691}} % 2231
  \author{Y.-T.~Lai\,\orcidlink{0000-0001-9553-3421}} % 2066
% \author{K.~Lalwani\,\orcidlink{0000-0002-7294-396X}} % 2142
  \author{T.~Lam\,\orcidlink{0000-0001-9128-6806}} % 2729
% \author{J.~S.~Lange\,\orcidlink{0000-0003-0234-0474}} % 2277
  \author{M.~Laurenza\,\orcidlink{0000-0002-7400-6013}} % 10223
% \author{I.~S.~Lee\,\orcidlink{0000-0002-7786-323X}} % 2422
% \author{J.~K.~Lee\,\orcidlink{0000-0001-6397-0723}} % 2190
  \author{S.~C.~Lee\,\orcidlink{0000-0002-9835-1006}} % 2544
  \author{D.~Levit\,\orcidlink{0000-0001-5789-6205}} % 2507
% \author{P.~Lewis\,\orcidlink{0000-0002-5991-622X}} % 2582
% \author{C.~H.~Li\,\orcidlink{0000-0002-3240-4523}} % 2325
% \author{J.~Li\,\orcidlink{0000-0001-5520-5394}} % 11064
  \author{L.~K.~Li\,\orcidlink{0000-0002-7366-1307}} % 3263
% \author{S.~X.~Li\,\orcidlink{0000-0003-4669-1495}} % 2377
% \author{Y.~Li\,\orcidlink{0000-0002-4413-6247}} % 8083
% \author{Y.~B.~Li\,\orcidlink{0000-0002-9909-2851}} % 2573
  \author{L.~Li~Gioi\,\orcidlink{0000-0003-2024-5649}} % 2495
  \author{J.~Libby\,\orcidlink{0000-0002-1219-3247}} % 2262
  \author{K.~Lieret\,\orcidlink{0000-0003-2792-7511}} % 2268
  \author{Y.-R.~Lin\,\orcidlink{0000-0003-0864-6693}} % 9323
% \author{Z.~Liptak\,\orcidlink{0000-0002-6491-8131}} % 3565
  \author{D.~Liventsev\,\orcidlink{0000-0003-3416-0056}} % 2578
% \author{T.~Luo\,\orcidlink{0000-0001-5139-5784}} % 3268
  \author{Y.~Ma\,\orcidlink{0000-0001-8412-8308}} % 16883
% \author{J.~MacNaughton\,\orcidlink{-}} % -550
% \author{A.~Martini\,\orcidlink{0000-0003-1161-4983}} % 2336
  \author{M.~Masuda\,\orcidlink{0000-0002-7109-5583}} % 2238
% \author{T.~Matsuda\,\orcidlink{0000-0003-4673-570X}} % 5543
  \author{D.~Matvienko\,\orcidlink{0000-0002-2698-5448}} % 2351
  \author{S.~K.~Maurya\,\orcidlink{0000-0002-7764-5777}} % 9763
  \author{F.~Meier\,\orcidlink{0000-0002-6088-0412}} % 3103
  \author{M.~Merola\,\orcidlink{0000-0002-7082-8108}} % 2456
  \author{F.~Metzner\,\orcidlink{0000-0002-0128-264X}} % 2296
% \author{K.~Miyabayashi\,\orcidlink{0000-0003-4352-734X}} % 2327
% \author{H.~Miyake\,\orcidlink{0000-0002-7079-8236}} % 2452
% \author{H.~Miyata\,\orcidlink{0000-0002-1026-2894}} % 2071
  \author{R.~Mizuk\,\orcidlink{0000-0002-2209-6969}} % 2483
% \author{G.~B.~Mohanty\,\orcidlink{0000-0001-6850-7666}} % 2278
% \author{H.~K.~Moon\,\orcidlink{0000-0001-5213-6477}} % 2304
% \author{T.~J.~Moon\,\orcidlink{0000-0001-9886-8534}} % 2397
% \author{H.-G.~Moser\,\orcidlink{0000-0003-3579-9951}} % 2120
% \author{M.~Mrvar\,\orcidlink{0000-0001-6388-3005}} % 2527
% \author{T.~M\"uller\,\orcidlink{0000-0003-4337-0098}} % 2165
  \author{R.~Mussa\,\orcidlink{0000-0002-0294-9071}} % 2372
  \author{I.~Nakamura\,\orcidlink{0000-0002-7640-5456}} % 3463
% \author{K.~R.~Nakamura\,\orcidlink{0000-0001-7012-7355}} % 2417
% \author{E.~Nakano\,\orcidlink{0000-0003-2282-5217}} % 2554
% \author{T.~Nakano\,\orcidlink{0000-0003-3157-5328}} % 2983
  \author{M.~Nakao\,\orcidlink{0000-0001-8424-7075}} % 2498
% \author{H.~Nakayama\,\orcidlink{0000-0002-2030-9967}} % 2232
% \author{H.~Nakazawa\,\orcidlink{0000-0003-1684-6628}} % 2335
% \author{D.~Narwal\,\orcidlink{0000-0001-6585-7767}} % 7223
% \author{Z.~Natkaniec\,\orcidlink{0000-0003-0486-9291}} % 3923
  \author{A.~Natochii\,\orcidlink{0000-0002-1076-814X}} % 12063
  \author{L.~Nayak\,\orcidlink{0000-0002-7739-914X}} % 9464
% \author{M.~Nayak\,\orcidlink{0000-0002-2572-4692}} % 2371
% \author{C.~Niebuhr\,\orcidlink{0000-0002-4375-9741}} % 2477
% \author{M.~Niiyama\,\orcidlink{0000-0003-1746-586X}} % 2063
  \author{N.~K.~Nisar\,\orcidlink{0000-0001-9562-1253}} % 2522
  \author{S.~Nishida\,\orcidlink{0000-0001-6373-2346}} % 2571
% \author{K.~Nishimura\,\orcidlink{0000-0001-8818-8922}} % 3063
  \author{K.~Ogawa\,\orcidlink{0000-0003-2220-7224}} % 2430
  \author{S.~Ogawa\,\orcidlink{0000-0002-7310-5079}} % 6263
% \author{S.~Okuno\,\orcidlink{-}} % -164
% \author{S.~L.~Olsen\,\orcidlink{0000-0002-6388-9885}} % 4563
  \author{H.~Ono\,\orcidlink{0000-0003-4486-0064}} % 2160
% \author{Y.~Onuki\,\orcidlink{0000-0002-1646-6847}} % 2331
  \author{P.~Oskin\,\orcidlink{0000-0002-7524-0936}} % 9623
% \author{H.~Ozaki\,\orcidlink{0000-0001-6901-1881}} % 2984
  \author{P.~Pakhlov\,\orcidlink{0000-0001-7426-4824}} % 2221
  \author{G.~Pakhlova\,\orcidlink{0000-0001-7518-3022}} % 2188
% \author{T.~Pang\,\orcidlink{0000-0003-1204-0846}} % 2114
  \author{S.~Pardi\,\orcidlink{0000-0001-7994-0537}} % 2532
% \author{H.~Park\,\orcidlink{0000-0001-6087-2052}} % 2284
  \author{J.~Park\,\orcidlink{0000-0001-6520-0028}} % 18203
  \author{S.-H.~Park\,\orcidlink{0000-0001-6019-6218}} % 2509
  \author{A.~Passeri\,\orcidlink{0000-0003-4864-3411}} % 2116
  \author{S.~Patra\,\orcidlink{0000-0002-4114-1091}} % 3123
  \author{S.~Paul\,\orcidlink{0000-0002-8813-0437}} % 2131
  \author{T.~K.~Pedlar\,\orcidlink{0000-0001-9839-7373}} % 2421
  \author{R.~Pestotnik\,\orcidlink{0000-0003-1804-9470}} % 2476
% \author{F.~Pham\,\orcidlink{0000-0003-0608-2302}} % 2963
  \author{L.~E.~Piilonen\,\orcidlink{0000-0001-6836-0748}} % 2346
  \author{T.~Podobnik\,\orcidlink{0000-0002-6131-819X}} % 11223
% \author{V.~Popov\,\orcidlink{0000-0003-0208-2583}} % 2096
% \author{S.~Prell\,\orcidlink{0000-0002-0195-8005}} % 12743
  \author{E.~Prencipe\,\orcidlink{0000-0002-9465-2493}} % 2219
  \author{M.~T.~Prim\,\orcidlink{0000-0002-1407-7450}} % 2501
% \author{M.~V.~Purohit\,\orcidlink{0000-0002-8381-8689}} % 2196
% \author{A.~Rabusov\,\orcidlink{0000-0001-8189-7398}} % 2355
% \author{M.~Ritter\,\orcidlink{0000-0001-6507-4631}} % 2580
% \author{M.~R\"{o}hrken\,\orcidlink{0000-0003-0654-2866}} % 11883
% \author{A.~Rostomyan\,\orcidlink{0000-0003-1839-8152}} % 2481
  \author{N.~Rout\,\orcidlink{0000-0002-4310-3638}} % 2965
% \author{M.~Rozanska\,\orcidlink{0000-0003-2651-5021}} % 2205
  \author{G.~Russo\,\orcidlink{0000-0001-5823-4393}} % 2388
% \author{D.~Sahoo\,\orcidlink{0000-0002-5600-9413}} % 2110
% \author{Y.~Sakai\,\orcidlink{0000-0001-9163-3409}} % 2175
% \author{M.~Salehi\,\orcidlink{-}} % 2127
  \author{S.~Sandilya\,\orcidlink{0000-0002-4199-4369}} % 2286
  \author{A.~Sangal\,\orcidlink{0000-0001-5853-349X}} % 2384
  \author{L.~Santelj\,\orcidlink{0000-0003-3904-2956}} % 2185
% \author{T.~Sanuki\,\orcidlink{0000-0002-4537-5899}} % 6783
  \author{V.~Savinov\,\orcidlink{0000-0002-9184-2830}} % 2292
% \author{P.~Schmolz\,\orcidlink{-}} % 4685
% \author{O.~Schneider\,\orcidlink{-}} % -198
  \author{G.~Schnell\,\orcidlink{0000-0002-7336-3246}} % 12204
% \author{J.~Schueler\,\orcidlink{0000-0002-2722-6953}} % 2824
  \author{C.~Schwanda\,\orcidlink{0000-0003-4844-5028}} % 2108
% \author{A.~J.~Schwartz\,\orcidlink{0000-0002-7310-1983}} % 2162
% \author{B.~Schwenker\,\orcidlink{0000-0002-7120-3732}} % 2405
% \author{R.~Seidl\,\orcidlink{0000-0002-6552-6973}} % -115
  \author{Y.~Seino\,\orcidlink{0000-0002-8378-4255}} % 2517
  \author{K.~Senyo\,\orcidlink{0000-0002-1615-9118}} % 2987
% \author{O.~Seon\,\orcidlink{-}} % 2581
  \author{M.~E.~Sevior\,\orcidlink{0000-0002-4824-101X}} % 2328
  \author{W.~Shan\,\orcidlink{0000-0003-2811-2218}} % 11943
  \author{M.~Shapkin\,\orcidlink{0000-0002-4098-9592}} % 2460
  \author{C.~Sharma\,\orcidlink{0000-0002-1312-0429}} % 11584
% \author{V.~Shebalin\,\orcidlink{0000-0003-1012-0957}} % 2339
% \author{C.~P.~Shen\,\orcidlink{0000-0002-9012-4618}} % 2464
% \author{H.~Shibuya\,\orcidlink{0000-0002-0197-6270}} % 2234
  \author{J.-G.~Shiu\,\orcidlink{0000-0002-8478-5639}} % 2412
% \author{B.~Shwartz\,\orcidlink{0000-0002-1456-1496}} % 2122
% \author{A.~Sibidanov\,\orcidlink{0000-0001-8805-4895}} % 2419
% \author{F.~Simon\,\orcidlink{0000-0002-5978-0289}} % 2164
  \author{J.~B.~Singh\,\orcidlink{0000-0001-9029-2462}} % 2903
% \author{R.~Sinha\,\orcidlink{-}} % 3423
% \author{K.~Smith\,\orcidlink{0000-0003-0446-9474}} % 2243
  \author{A.~Sokolov\,\orcidlink{0000-0002-9420-0091}} % 2521
% \author{Y.~Soloviev\,\orcidlink{0000-0003-1136-2827}} % 2479
  \author{E.~Solovieva\,\orcidlink{0000-0002-5735-4059}} % 2398
% \author{S.~Stani\v{c}\,\orcidlink{0000-0003-3344-8381}} % 3383
  \author{M.~Stari\v{c}\,\orcidlink{0000-0001-8751-5944}} % 2326
% \author{Z.~S.~Stottler\,\orcidlink{0000-0002-1898-5333}} % 2267
  \author{J.~F.~Strube\,\orcidlink{0000-0001-7470-9301}} % 2451
% \author{J.~Stypula\,\orcidlink{0000-0002-5844-7476}} % 2368
  \author{M.~Sumihama\,\orcidlink{0000-0002-8954-0585}} % 4243
% \author{K.~Sumisawa\,\orcidlink{0000-0001-7003-7210}} % 2583
% \author{T.~Sumiyoshi\,\orcidlink{0000-0002-0486-3896}} % 4184
  \author{W.~Sutcliffe\,\orcidlink{0000-0002-9795-3582}} % 3784
% \author{S.~Y.~Suzuki\,\orcidlink{0000-0002-7135-4901}} % 2496
  \author{M.~Takizawa\,\orcidlink{0000-0001-8225-3973}} % 2437
% \author{U.~Tamponi\,\orcidlink{0000-0001-6651-0706}} % 2366
% \author{S.~Tanaka\,\orcidlink{0000-0002-6029-6216}} % 2530
% \author{S.~S.~Tang\,\orcidlink{0000-0001-6564-0445}} % 12003
  \author{K.~Tanida\,\orcidlink{0000-0002-8255-3746}} % 3803
% \author{N.~Taniguchi\,\orcidlink{0000-0002-1462-0564}} % 2285
% \author{Y.~Tao\,\orcidlink{0000-0002-9186-2591}} % 2362
% \author{G.~N.~Taylor\,\orcidlink{-}} % -220
  \author{F.~Tenchini\,\orcidlink{0000-0003-3469-9377}} % 2546
% \author{Y.~Teramoto\,\orcidlink{0000-0002-1738-6697}} % -349
% \author{A.~Thampi\,\orcidlink{-}} % 7403
  \author{R.~Tiwary\,\orcidlink{0000-0002-5887-1883}} % 10403
  \author{K.~Trabelsi\,\orcidlink{0000-0001-6567-3036}} % 2369
% \author{T.~Tsuboyama\,\orcidlink{0000-0002-4575-1997}} % 2361
% \author{N.~Tsuzuki\,\orcidlink{0000-0003-1141-1908}} % 2352
  \author{M.~Uchida\,\orcidlink{0000-0003-4904-6168}} % 2370
% \author{I.~Ueda\,\orcidlink{0000-0002-6833-4344}} % 2519
% \author{S.~Uehara\,\orcidlink{0000-0001-7377-5016}} % 2586
% \author{T.~Uglov\,\orcidlink{0000-0002-4944-1830}} % 2252
  \author{Y.~Unno\,\orcidlink{0000-0003-3355-765X}} % 2420
% \author{K.~Uno\,\orcidlink{0000-0002-2209-8198}} % 14963
  \author{S.~Uno\,\orcidlink{0000-0002-3401-0480}} % 2149
% \author{P.~Urquijo\,\orcidlink{0000-0002-0887-7953}} % 2302
% \author{Y.~Ushiroda\,\orcidlink{0000-0003-3174-403X}} % 2317
  \author{Y.~Usov\,\orcidlink{0000-0003-3144-2920}} % 5003
  \author{S.~E.~Vahsen\,\orcidlink{0000-0003-1685-9824}} % 2251
  \author{G.~Varner\,\orcidlink{0000-0002-0302-8151}} % 2119
  \author{K.~E.~Varvell\,\orcidlink{0000-0003-1017-1295}} % 2545
% \author{A.~Vinokurova\,\orcidlink{0000-0003-4220-8056}} % 2289
% \author{V.~Vorobyev\,\orcidlink{0000-0002-6660-868X}} % 2298
% \author{A.~Vossen\,\orcidlink{0000-0003-0983-4936}} % 2249
% \author{E.~Waheed\,\orcidlink{0000-0001-7774-0363}} % 2226
% \author{B.~Wang\,\orcidlink{0000-0001-6136-6952}} % 2569
% \author{C.~H.~Wang\,\orcidlink{0000-0001-6760-9839}} % 2224
  \author{D.~Wang\,\orcidlink{0000-0003-1485-2143}} % 10003
  \author{E.~Wang\,\orcidlink{0000-0001-6391-5118}} % 10983
% \author{X.~L.~Wang\,\orcidlink{0000-0001-5805-1255}} % 2076
% \author{M.~Watanabe\,\orcidlink{0000-0001-6917-6694}} % 2309
% \author{Y.~Watanabe\,\orcidlink{-}} % -165
  \author{S.~Watanuki\,\orcidlink{0000-0002-5241-6628}} % 6843
% \author{S.~Wehle\,\orcidlink{0000-0002-6168-1829}} % 2489
  \author{O.~Werbycka\,\orcidlink{0000-0002-0614-8773}} % 6123
% \author{E.~Widmann\,\orcidlink{-}} % -509
% \author{J.~Wiechczynski\,\orcidlink{0000-0002-3151-6072}} % 2604
  \author{E.~Won\,\orcidlink{0000-0002-4245-7442}} % 2410
% \author{X.~Xu\,\orcidlink{0000-0001-5096-1182}} % 4923
  \author{B.~D.~Yabsley\,\orcidlink{0000-0002-2680-0474}} % 3645
% \author{S.~Yamada\,\orcidlink{0000-0002-8858-9336}} % 2492
% \author{H.~Yamamoto\,\orcidlink{-}} % 2964
  \author{W.~Yan\,\orcidlink{0000-0003-0713-0871}} % 2094
  \author{S.~B.~Yang\,\orcidlink{0000-0002-9543-7971}} % 2374
% \author{H.~Ye\,\orcidlink{0000-0003-0552-5490}} % 2537
% \author{J.~Yelton\,\orcidlink{0000-0001-8840-3346}} % 2067
  \author{J.~H.~Yin\,\orcidlink{0000-0002-1479-9349}} % 2365
% \author{Y.~Yook\,\orcidlink{0000-0002-4912-048X}} % 2453
  \author{C.~Z.~Yuan\,\orcidlink{0000-0002-1652-6686}} % 2088
  \author{L.~Yuan\,\orcidlink{0000-0002-6719-5397}} % 14003
  \author{Y.~Yusa\,\orcidlink{0000-0002-4001-9748}} % 2357
% \author{Y.~Zhai\,\orcidlink{0000-0001-7207-5122}} % 12703
% \author{J.~Zhang\,\orcidlink{0000-0001-6535-0659}} % 2349
  \author{Z.~P.~Zhang\,\orcidlink{0000-0001-6140-2044}} % 5363
  \author{V.~Zhilich\,\orcidlink{0000-0002-0907-5565}} % 4703
  \author{V.~Zhukova\,\orcidlink{0000-0002-8253-641X}} % 2387
% \author{V.~Zhulanov\,\orcidlink{0000-0002-0306-9199}} % 4983
\collaboration{The Belle Collaboration}


==> pub648.tex <==
%%% Paper:    B0 to p Sigma0-bar pi-
%%% Journal:  Physical Review D
%%% Contacts: C.Y. Chang, M.Z. Wang
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{pub648} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen}
\newcommand{\instBeihang}{Beihang University, Beijing 100191}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000}
\newcommand{\instEPFL}{\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne 1015}
\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763}
\newcommand{\instHNU}{Henan Normal University, Xinxiang 453007}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530}
\newcommand{\instHUNNU}{Hunan Normal University, Changsha 410081}
\newcommand{\instIKERBASQUE}{IKERBASQUE, Basque Foundation for Science, 48013 Bilbao}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049}
\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195}
\newcommand{\instKanagawa}{Kanagawa University, Yokohama 221-8686}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe}
\newcommand{\instKAU}{Department of Physics, Faculty of Science, King Abdulaziz University, Jeddah 21589}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich}
\newcommand{\instSMI}{Stefan Meyer Institute for Subatomic Physics, Vienna 1090}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506}
\newcommand{\instNCU}{National Central University, Chung-li 32054}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181}
\newcommand{\instNDU}{Nippon Dental University, Niigata 951-8580}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014}
\newcommand{\instPeking}{Peking University, Beijing 100871}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198}
\newcommand{\instRIKENBNL}{RIKEN BNL Research Center, Upton, New York 11973}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978}
\newcommand{\instSEU}{Southeast University, Nanjing 211189}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana}
\newcommand{\instSKKU}{Sungkyunkwan University, Suwon 16419}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching}
\newcommand{\instTelAviv}{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978}
\newcommand{\instToho}{Toho University, Funabashi 274-8510}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay}
\newcommand{\instBilbao}{Department of Physics \& EHU Quantum Center, University of the Basque Country UPV/EHU, 48080 Bilbao}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292}
\newcommand{\instMalaya}{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
\newcommand{\instUSTC}{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583}
\newcommand{\instUtkal}{Utkal University, Bhubaneswar 751004}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722}
%%%\affiliation{\instGoettingen}
\affiliation{\instBeihang}
\affiliation{\instBNL}
\affiliation{\instBINP}
%%%\affiliation{\instCMU}
\affiliation{\instPrague}
%%%\affiliation{\instChiba}
\affiliation{\instChonnam}
\affiliation{\instCAU}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
%%%\affiliation{\instEPFL}
%%%\affiliation{\instJuelich}
\affiliation{\instFuJen}
%%%\affiliation{\instFudan}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
%%%\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
%%%\affiliation{\instHNU}
\affiliation{\instKEK}
\affiliation{\instJPARC}
%%%\affiliation{\instHiroshima}
\affiliation{\instHUNNU}
\affiliation{\instIKERBASQUE}
\affiliation{\instNapoliINFN}
\affiliation{\instPisaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instIISER}
%%%\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instISU}
\affiliation{\instJAEA}
%%%\affiliation{\instKanagawa}
\affiliation{\instKarlsruhe}
\affiliation{\instKAU}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
%%%\affiliation{\instKSU}
\affiliation{\instKyungpook}
%%%\affiliation{\instLNNU}
\affiliation{\instGiessen}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instLMU}
%%%\affiliation{\instSMI}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
%%%\affiliation{\instNagoyaKMI}
\affiliation{\instNaraWu}
%%%\affiliation{\instNCU}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
%%%\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNDU}
\affiliation{\instNSU}
%%%\affiliation{\instOkinawa}
\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
%%%\affiliation{\instPeking}
\affiliation{\instMPP}
%%%\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKENBNL}
%%%\affiliation{\instSeoul}
\affiliation{\instSPU}
%%%\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instSEU}
\affiliation{\instLjubljanaJSI}
\affiliation{\instSKKU}
\affiliation{\instTata}
\affiliation{\instTUM}
%%%\affiliation{\instTelAviv}
\affiliation{\instToho}
%%%\affiliation{\instTohoku}
\affiliation{\instTitech}
%%%\affiliation{\instTokyoMetropolitan}
\affiliation{\instNapoliUNIV}
\affiliation{\instPisaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instIJCLab}
\affiliation{\instBilbao}
\affiliation{\instBonn}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
\affiliation{\instHawaii}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
%%%\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
%%%\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSydney}
\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instEri}
%%%\affiliation{\instIPMU}
%%%\affiliation{\instUtkal}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instYamagata}
\affiliation{\instYonsei}
  \author{C.-Y.~Chang}\affiliation{\instNTUTaiwan} % Taiwan
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % Taiwan
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~Adamczyk}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % Korea
  \author{H.~Aihara}\affiliation{\instUTokyo} % Tokyo
  \author{S.~Al~Said}\affiliation{\instTabuk}\affiliation{\instKAU} % Tabuk
  \author{D.~M.~Asner}\affiliation{\instBNL} % BNL
  \author{H.~Atmacan}\affiliation{\instCincinnati} % Cincinnati
% \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{T.~Aushev}\affiliation{\instHSE} % HSE
  \author{R.~Ayad}\affiliation{\instTabuk} % Tabuk
% \author{T.~Aziz}\affiliation{\instTata} % Tata
  \author{V.~Babu}\affiliation{\instIJCLab} % IJCLab
% \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % IITB
% \author{A.~M.~Bakich}\affiliation{\instSydney} % Sydney
% \author{Y.~Ban}\affiliation{\instPeking} % Peking
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % Louisville
% \author{E.~Barberio}\affiliation{\instMelbourne} % Melbourne
% \author{M.~Barrett}\affiliation{\instKEK} % KEK
  \author{M.~Bauer}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{P.~Behera}\affiliation{\instIITMadras} % IITM
  \author{K.~Belous}\affiliation{\instIHEPRussia} % Protvino
  \author{J.~Bennett}\affiliation{\instMississippi} % Mississippi
  \author{F.~Bernlochner}\affiliation{\instBonn} % Bonn
  \author{M.~Bessner}\affiliation{\instHawaii} % Hawaii
% \author{D.~Besson}\affiliation{\instMEPhI} % MEPhI
% \author{V.~Bhardwaj}\affiliation{\instIISER} % IISERM
% \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % IITG
  \author{T.~Bilka}\affiliation{\instPrague} % Charles
% \author{S.~Bilokin}\affiliation{\instLMU} % LMU
  \author{D.~Biswas}\affiliation{\instLouisville} % Louisville
% \author{T.~Bloomfield}\affiliation{\instKEK} % KEK
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{D.~Bodrov}\affiliation{\instHSE} % HSE
% \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{G.~Bonvicini}\affiliation{\instWayneState} % WayneState
  \author{J.~Borah}\affiliation{\instIITGuwahati} % IITG
  \author{A.~Bozek}\affiliation{\instKrakow} % Krakow
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % RomaTre
  \author{T.~E.~Browder}\affiliation{\instHawaii} % Hawaii
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % RomaTre
  \author{M.~Campajola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{L.~Cao}\affiliation{\instDESY} % DESY
  \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % Charles
  \author{M.-C.~Chang}\affiliation{\instFuJen} % FuJen
% \author{P.~Chang}\affiliation{\instNTUTaiwan} % Taiwan
% \author{V.~Chekelian}\affiliation{\instMPP} % MPI
% \author{A.~Chen}\affiliation{\instNCU} % NCU
% \author{C.~Chen}\affiliation{\instISU} % ISU
% \author{Y.~Chen}\affiliation{\instUSTC} % USTC
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % Taiwan
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % Hanyang
  \author{K.~Chilikin}\affiliation{\instBINP} % BINP
  \author{H.~E.~Cho}\affiliation{\instHanyang} % Hanyang
  \author{K.~Cho}\affiliation{\instKISTI} % KISTI
  \author{S.-J.~Cho}\affiliation{\instYonsei} % Yonsei
  \author{S.-K.~Choi}\affiliation{\instCAU} % CAU
  \author{Y.~Choi}\affiliation{\instSKKU} % Sungkyunkwan
  \author{S.~Choudhury}\affiliation{\instISU} % ISU
  \author{D.~Cinabro}\affiliation{\instWayneState} % WayneState
% \author{J.~Cochran}\affiliation{\instISU} % ISU
% \author{S.~Cunliffe}\affiliation{\instDESY} % DESY
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % TMU
  \author{S.~Das}\affiliation{\instMNITJaipur} % MNIT
% \author{N.~Dash}\affiliation{\instIITMadras} % IITM
% \author{G.~de~Marino}\affiliation{\instIJCLab} % IJCLab
  \author{G.~De~Nardo}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{G.~De~Pietro}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{R.~Dhamija}\affiliation{\instIITHyderabad} % IITH
  \author{F.~Di~Capua}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
% \author{J.~Dingfelder}\affiliation{\instBonn} % Bonn
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % Charles
  \author{T.~V.~Dong}\affiliation{\instITAR} % DuyTan
% \author{D.~Dossett}\affiliation{\instMelbourne} % Melbourne
  \author{S.~Dubey}\affiliation{\instHawaii} % Hawaii
  \author{P.~Ecker}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{M.~Feindt}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{T.~Ferber}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % Melbourne
% \author{A.~Frey}\affiliation{\instGoettingen} % Goettingen
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % PNNL
% \author{R.~Garg}\affiliation{\instCMU} % CMU
  \author{V.~Gaur}\affiliation{\instUPES} % UPES
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{A.~Giri}\affiliation{\instIITHyderabad} % IITH
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{G.~Gong}\affiliation{\instUSTC} % USTC
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % RomaTre
% \author{D.~Greenwald}\affiliation{\instTUM} % TUM
  \author{T.~Gu}\affiliation{\instPittsburgh} % Pittsburgh
  \author{Y.~Guan}\affiliation{\instCincinnati} % Cincinnati
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % PNNL
% \author{H.~Haigh}\affiliation{\instHEPHYVienna} % Vienna
  \author{S.~Halder}\affiliation{\instTata} % Tata
% \author{X.~Han}\affiliation{\instBeihang} % Beihang
% \author{K.~Hara}\affiliation{\instKEK} % KEK
  \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{O.~Hartbrich}\affiliation{\instHawaii} % Hawaii
  \author{K.~Hayasaka}\affiliation{\instNiigata} % Niigata
  \author{H.~Hayashii}\affiliation{\instNaraWu} % Nara
  \author{S.~Hazra}\affiliation{\instTata} % Tata
  \author{M.~T.~Hedges}\affiliation{\instBonn} % Bonn
  \author{D.~Herrmann}\affiliation{\instWayneState} % WayneState
% \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instDESY} % DESY
% \author{T.~Higuchi}\affiliation{\instIPMU} % IPMU
% \author{H.~Hirata}\affiliation{\instNagoya} % Nagoya
  \author{W.-S.~Hou}\affiliation{\instNTUTaiwan} % Taiwan
  \author{C.-L.~Hsu}\affiliation{\instSydney} % Sydney
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % Taiwan
% \author{T.~Iijima}\affiliation{\instNagoyaKMI}\affiliation{\instNagoya} % Nagoya
  \author{K.~Inami}\affiliation{\instNagoya} % Nagoya
% \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % Vienna
  \author{N.~Ipsita}\affiliation{\instIITHyderabad} % IITH
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % OsakaCity
  \author{Y.~Iwasaki}\affiliation{\instKEK} % KEK
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % TMU
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % Indiana
% \author{E.-J.~Jang}\affiliation{\instGyeongsang} % Gyeongsang
% \author{H.~B.~Jeon}\affiliation{\instKyungpook} % Kyungpook
% \author{Q.~P.~Ji}\affiliation{\instHNU} % HNU
  \author{S.~Jia}\affiliation{\instSEU} % SEU
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % Trieste
  \author{K.~K.~Joo}\affiliation{\instChonnam} % Chonnam
% \author{J.~Kahn}\affiliation{\instKarlsruhe} % Karlsruhe
% \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % TMU
% \author{D.~Kalita}\affiliation{\instIITGuwahati} % IITG
  \author{A.~B.~Kaliyar}\affiliation{\instHEPHYVienna} % Vienna
% \author{K.~H.~Kang}\affiliation{\instIPMU} % IPMU
% \author{S.~Kang}\affiliation{\instISU} % ISU
% \author{P.~Kapusta}\affiliation{\instKrakow} % Krakow
% \author{G.~Karyan}\affiliation{\instDESY} % DESY
% \author{Y.~Kato}\affiliation{\instNagoya} % Nagoya
% \author{H.~Kawai}\affiliation{\instChiba} % Chiba
  \author{T.~Kawasaki}\affiliation{\instKitasato} % Kitasato
% \author{H.~Kichimi}\affiliation{\instKEK} % KEK
  \author{C.~Kiesling}\affiliation{\instMPP} % MPI
  \author{C.~H.~Kim}\affiliation{\instHanyang} % Hanyang
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % Soongsil
% \author{H.~J.~Kim}\affiliation{\instKyungpook} % Kyungpook
  \author{K.-H.~Kim}\affiliation{\instKISTI} % KISTI
% \author{K.~T.~Kim}\affiliation{\instKoreaUnivKU} % Korea
% \author{S.~K.~Kim}\affiliation{\instSeoul} % Seoul
% \author{Y.~J.~Kim}\affiliation{\instKoreaUnivKU} % Korea
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % Yonsei
% \author{T.~D.~Kimmel}\affiliation{\instVPI} % VPI
% \author{H.~Kindo}\affiliation{\instVPI}\affiliation{\instKEK} % VPI
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % Cincinnati
% \author{C.~Kleinwort}\affiliation{\instDESY} % DESY
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % Charles
% \author{I.~Komarov}\affiliation{\instDESY} % DESY
  \author{T.~Konno}\affiliation{\instKitasato} % Kitasato
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % Ljubljana
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{R.~Kroeger}\affiliation{\instMississippi} % Mississippi
% \author{J.-F.~Krohn}\affiliation{\instMelbourne} % Melbourne
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{T.~Kuhr}\affiliation{\instLMU} % LMU
  \author{M.~Kumar}\affiliation{\instIISER} % IISERM
% \author{R.~Kumar}\affiliation{\instPanjabPAU} % Punjab
  \author{K.~Kumara}\affiliation{\instMississippi} % Mississippi
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % TMU
% \author{E.~Kurihara}\affiliation{\instChiba} % Chiba
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % Charles
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % Yonsei
  \author{Y.-T.~Lai}\affiliation{\instKEK} % KEK
% \author{K.~Lalwani}\affiliation{\instMNITJaipur} % MNIT
  \author{T.~Lam}\affiliation{\instVPI} % VPI
% \author{J.~S.~Lange}\affiliation{\instGiessen} % Giessen
  \author{M.~Laurenza}\affiliation{\instRomaTreINFN}\affiliation{\instRomaTreUNIV} % RomaTre
% \author{I.~S.~Lee}\affiliation{\instHanyang} % Hanyang
% \author{J.~K.~Lee}\affiliation{\instSeoul} % Seoul
  \author{S.~C.~Lee}\affiliation{\instKyungpook} % Kyungpook
  \author{D.~Levit}\affiliation{\instKEK} % KEK
% \author{P.~Lewis}\affiliation{\instBonn} % Bonn
% \author{C.~H.~Li}\affiliation{\instLNNU} % LNNU
% \author{J.~Li}\affiliation{\instKyungpook} % Kyungpook
  \author{L.~K.~Li}\affiliation{\instCincinnati} % Cincinnati
% \author{S.~X.~Li}\affiliation{\instFudan} % Fudan
% \author{Y.~Li}\affiliation{\instFudan} % Fudan
% \author{Y.~B.~Li}\affiliation{\instFudan} % Fudan
  \author{L.~Li~Gioi}\affiliation{\instMPP} % MPI
  \author{J.~Libby}\affiliation{\instIITMadras} % IITM
  \author{K.~Lieret}\affiliation{\instLMU} % LMU
  \author{Y.-R.~Lin}\affiliation{\instNTUTaiwan} % Taiwan
% \author{Z.~Liptak}\affiliation{\instHiroshima} % Hiroshima
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % WayneState
% \author{T.~Luo}\affiliation{\instFudan} % Fudan
  \author{Y.~Ma}\affiliation{\instRIKENMSL} % NPC
% \author{J.~MacNaughton}\affiliation{\instUOM} % NPC
% \author{A.~Martini}\affiliation{\instDESY} % DESY
  \author{M.~Masuda}\affiliation{\instEri}\affiliation{\instRCNP} % NPC
% \author{T.~Matsuda}\affiliation{\instUOM} % NPC
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % IITG
  \author{F.~Meier}\affiliation{\instDuke} % Duke
  \author{M.~Merola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % Napoli
  \author{F.~Metzner}\affiliation{\instBonn} % Bonn
% \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % Nara
% \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Miyata}\affiliation{\instNiigata} % Niigata
  \author{R.~Mizuk}\affiliation{\instHSE} % HSE
% \author{G.~B.~Mohanty}\affiliation{\instTata} % Tata
% \author{H.~K.~Moon}\affiliation{\instKoreaUnivKU} % Korea
% \author{T.~J.~Moon}\affiliation{\instSeoul} % Seoul
% \author{H.-G.~Moser}\affiliation{\instMPP} % MPI
% \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % Vienna
% \author{T.~M\"uller}\affiliation{\instKarlsruhe} % Karlsruhe
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % Torino
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~R.~Nakamura}\affiliation{\instKEK} % KEK
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % OsakaCity
% \author{T.~Nakano}\affiliation{\instRCNP} % NPC
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % Taiwan
% \author{D.~Narwal}\affiliation{\instIITGuwahati} % IITG
% \author{Z.~Natkaniec}\affiliation{\instKrakow} % Krakow
  \author{A.~Natochii}\affiliation{\instHawaii} % Hawaii
  \author{L.~Nayak}\affiliation{\instIITHyderabad} % IITH
% \author{M.~Nayak}\affiliation{\instTelAviv} % TelAviv
% \author{C.~Niebuhr}\affiliation{\instDESY} % DESY
% \author{M.~Niiyama}\affiliation{\instKSU} % NPC
  \author{N.~K.~Nisar}\affiliation{\instBNL} % BNL
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{K.~Nishimura}\affiliation{\instHawaii} % Hawaii
  \author{K.~Ogawa}\affiliation{\instNiigata} % Niigata
  \author{S.~Ogawa}\affiliation{\instToho} % Toho
% \author{S.~Okuno}\affiliation{\instKanagawa} % Kanagawa
% \author{S.~L.~Olsen}\affiliation{\instCAU} % CAU
  \author{H.~Ono}\affiliation{\instNDU}\affiliation{\instNiigata} % NihonDental
% \author{Y.~Onuki}\affiliation{\instUTokyo} % Tokyo
  \author{P.~Oskin}\affiliation{\instIJCLab} % IJCLab
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{P.~Pakhlov}\affiliation{\instHSE} % HSE
  \author{G.~Pakhlova}\affiliation{\instHSE} % HSE
% \author{T.~Pang}\affiliation{\instPittsburgh} % Pittsburgh
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % Napoli
% \author{H.~Park}\affiliation{\instKyungpook} % Kyungpook
  \author{J.~Park}\affiliation{\instYonsei} % Yonsei
  \author{S.-H.~Park}\affiliation{\instKEK} % KEK
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % RomaTre
  \author{S.~Patra}\affiliation{\instLouisville} % Louisville
  \author{S.~Paul}\affiliation{\instTUM}\affiliation{\instMPP} % TUM
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % Luther
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{F.~Pham}\affiliation{\instMelbourne} % Melbourne
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % VPI
  \author{T.~Podobnik}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{V.~Popov}\affiliation{\instHSE} % HSE
% \author{S.~Prell}\affiliation{\instISU} % ISU
  \author{E.~Prencipe}\affiliation{\instGiessen} % Giessen
  \author{M.~T.~Prim}\affiliation{\instBonn} % Bonn
% \author{M.~V.~Purohit}\affiliation{\instOkinawa} % OIST
% \author{A.~Rabusov}\affiliation{\instTUM} % TUM
% \author{M.~Ritter}\affiliation{\instLMU} % LMU
% \author{M.~R\"{o}hrken}\affiliation{\instDESY} % DESY
% \author{A.~Rostomyan}\affiliation{\instDESY} % DESY
  \author{N.~Rout}\affiliation{\instTriesteINFN} % Trieste
% \author{M.~Rozanska}\affiliation{\instKrakow} % Krakow
  \author{G.~Russo}\affiliation{\instNapoliUNIV} % Napoli
% \author{D.~Sahoo}\affiliation{\instISU} % ISU
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{M.~Salehi}\affiliation{\instMalaya}\affiliation{\instLMU} % Malaya
  \author{S.~Sandilya}\affiliation{\instIITHyderabad} % IITH
  \author{A.~Sangal}\affiliation{\instCincinnati} % Cincinnati
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{T.~Sanuki}\affiliation{\instTohoku} % Tohoku
  \author{V.~Savinov}\affiliation{\instPittsburgh} % Pittsburgh
% \author{P.~Schmolz}\affiliation{\instLMU} % LMU
% \author{O.~Schneider}\affiliation{\instEPFL} % Lausanne
  \author{G.~Schnell}\affiliation{\instBilbao}\affiliation{\instIKERBASQUE} % Bilbao
% \author{J.~Schueler}\affiliation{\instHawaii} % Hawaii
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % Vienna
% \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % Cincinnati
% \author{B.~Schwenker}\affiliation{\instGoettingen} % Goettingen
% \author{R.~Seidl}\affiliation{\instRIKENBNL} % RIKEN
  \author{Y.~Seino}\affiliation{\instNiigata} % Niigata
  \author{K.~Senyo}\affiliation{\instYamagata} % Yamagata
% \author{O.~Seon}\affiliation{\instNagoya} % Nagoya
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % Melbourne
  \author{W.~Shan}\affiliation{\instHUNNU} % HUNNU
  \author{M.~Shapkin}\affiliation{\instIHEPRussia} % Protvino
  \author{C.~Sharma}\affiliation{\instMNITJaipur} % MNIT
% \author{V.~Shebalin}\affiliation{\instHawaii} % Hawaii
% \author{C.~P.~Shen}\affiliation{\instFudan} % Fudan
% \author{H.~Shibuya}\affiliation{\instToho} % Toho
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % Taiwan
% \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{A.~Sibidanov}\affiliation{\instHawaii} % Hawaii
% \author{F.~Simon}\affiliation{\instMPP} % MPI
  \author{J.~B.~Singh}\affiliation{\instPanjab}\affiliation{\instUPES} % Panjab
% \author{R.~Sinha}\affiliation{\instChennai} % IMSC
% \author{K.~Smith}\affiliation{\instMelbourne} % Melbourne
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % Protvino
% \author{Y.~Soloviev}\affiliation{\instDESY} % DESY
  \author{E.~Solovieva}\affiliation{\instBINP} % BINP
% \author{S.~Stani\v{c}}\affiliation{\instNovaGorica} % NovaGorica
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{Z.~S.~Stottler}\affiliation{\instVPI} % VPI
  \author{J.~F.~Strube}\affiliation{\instPNNL} % PNNL
% \author{J.~Stypula}\affiliation{\instKrakow} % Krakow
  \author{M.~Sumihama}\affiliation{\instGifu}\affiliation{\instRCNP} % NPC
% \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNaraWu} % KEK
% \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % TMU
  \author{W.~Sutcliffe}\affiliation{\instBonn} % Bonn
% \author{S.~Y.~Suzuki}\affiliation{\instKEK} % KEK
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % NPC
% \author{U.~Tamponi}\affiliation{\instTorinoINFN} % Torino
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{S.~S.~Tang}\affiliation{\instFudan} % Fudan
  \author{K.~Tanida}\affiliation{\instJAEA} % NPC
% \author{N.~Taniguchi}\affiliation{\instKEK} % KEK
% \author{Y.~Tao}\affiliation{\instFlorida} % Florida
% \author{G.~N.~Taylor}\affiliation{\instMelbourne} % Melbourne
  \author{F.~Tenchini}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % Pisa
% \author{Y.~Teramoto}\affiliation{\instOsakaMetropolitan} % OsakaCity
% \author{A.~Thampi}\affiliation{\instJuelich} % Juelich
  \author{R.~Tiwary}\affiliation{\instTata} % Tata
  \author{K.~Trabelsi}\affiliation{\instIJCLab} % IJCLab
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{N.~Tsuzuki}\affiliation{\instNagoya} % Nagoya
  \author{M.~Uchida}\affiliation{\instTitech} % NPC
% \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{T.~Uglov}\affiliation{\instHSE} % HSE
  \author{Y.~Unno}\affiliation{\instHanyang} % Hanyang
% \author{K.~Uno}\affiliation{\instNiigata} % Niigata
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
% \author{P.~Urquijo}\affiliation{\instMelbourne} % Melbourne
% \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % KEK
  \author{Y.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % Hawaii
  \author{G.~Varner}\affiliation{\instHawaii} % Hawaii
  \author{K.~E.~Varvell}\affiliation{\instSydney} % Sydney
% \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
% \author{V.~Vorobyev}\affiliation{\instBINP} % BINP
% \author{A.~Vossen}\affiliation{\instDuke} % Duke
% \author{E.~Waheed}\affiliation{\instKEK} % KEK
% \author{B.~Wang}\affiliation{\instMPP} % MPI
% \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % NUU
  \author{D.~Wang}\affiliation{\instFlorida} % Florida
  \author{E.~Wang}\affiliation{\instPittsburgh} % Pittsburgh
% \author{X.~L.~Wang}\affiliation{\instFudan} % Fudan
% \author{M.~Watanabe}\affiliation{\instNiigata} % Niigata
% \author{Y.~Watanabe}\affiliation{\instKanagawa} % Kanagawa
  \author{S.~Watanuki}\affiliation{\instYonsei} % Yonsei
% \author{S.~Wehle}\affiliation{\instDESY} % DESY
  \author{O.~Werbycka}\affiliation{\instTriesteINFN} % Trieste
% \author{E.~Widmann}\affiliation{\instSMI} % Vienna
% \author{J.~Wiechczynski}\affiliation{\instKrakow} % Krakow
  \author{E.~Won}\affiliation{\instKoreaUnivKU} % Korea
% \author{X.~Xu}\affiliation{\instSoochow} % Soochow
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % Sydney
% \author{S.~Yamada}\affiliation{\instKEK} % KEK
% \author{H.~Yamamoto}\affiliation{\instTohoku} % Tohoku
  \author{W.~Yan}\affiliation{\instUSTC} % USTC
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % Korea
% \author{H.~Ye}\affiliation{\instDESY} % DESY
% \author{J.~Yelton}\affiliation{\instFlorida} % Florida
  \author{J.~H.~Yin}\affiliation{\instKoreaUnivKU} % Korea
% \author{Y.~Yook}\affiliation{\instIHEPChina} % IHEP
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % IHEP
  \author{L.~Yuan}\affiliation{\instBeihang} % Beihang
  \author{Y.~Yusa}\affiliation{\instNiigata} % Niigata
% \author{Y.~Zhai}\affiliation{\instISU} % ISU
% \author{J.~Zhang}\affiliation{\instIHEPChina} % IHEP
  \author{Z.~P.~Zhang}\affiliation{\instUSTC} % USTC
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
  \author{V.~Zhukova}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % Ljubljana
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % BINP
\collaboration{The Belle Collaboration}

